Smoothed Efficient Algorithms and Reductions for Network Coordination Games

Worst-case hardness results for most equilibrium computation problems have raised the need for beyond-worst-case analysis. To this end, we study the smoothed complexity of finding pure Nash equilibria in Network Coordination Games, a PLS-complete problem in the worst case. This is a potential game where the sequential-better-response algorithm is known to converge to a pure NE, albeit in exponential time. First, we prove polynomial (resp. quasi-polynomial) smoothed complexity when the underlying game graph is a complete (resp. arbitrary) graph, and every player has constantly many strategies. We note that the complete graph case is reminiscent of perturbing all parameters, a common assumption in most known smoothed analysis results. Second, we define a notion of smoothness-preserving reduction among search problems, and obtain reductions from $2$-strategy network coordination games to local-max-cut, and from $k$-strategy games (with arbitrary $k$) to local-max-cut up to two flips. The former together with the recent result of [BCC18] gives an alternate $O(n^8)$-time smoothed algorithm for the $2$-strategy case. This notion of reduction allows for the extension of smoothed efficient algorithms from one problem to another. For the first set of results, we develop techniques to bound the probability that an (adversarial) better-response sequence makes slow improvements on the potential. Our approach combines and generalizes the local-max-cut approaches of [ER14,ABPW17] to handle the multi-strategy case: it requires a careful definition of the matrix which captures the increase in potential, a tighter union bound on adversarial sequences, and balancing it with good enough rank bounds. We believe that the approach and notions developed herein could be of interest in addressing the smoothed complexity of other potential and/or congestion games.

==> Section-3-Version-Sun-Oct-28.tex <==
\label{sec:PrelOR}

In this section, we give a high-level overview of the proof method and formally state the results of the paper. 
The following sections {\color{red}\bf (Sec Numbers?)} provide the details for these proofs.
As discussed previously, our results are twofold: first, we extend pre-existing proof methods to directly show that the BRA terminates in smoothed polynomial time, and second, we introduce the notion of a smoothness-preserving reduction which allows us to give an alternative algorithm for 2-\nashcoord, and a conditional algorithm for $k$-\nashcoord.
We begin with a formal definition of the smoothed problem here:

\vspace*{-3pt}
\paragraph{Smoothed $k$-\nashcoord.}
Given a $k$-\netco represented by an undirected graph $G=(V,E)$ and an $(|E|k^2)$-dimensional payoff vector $A$, where each entry of $A$ is an independent random variable supported on the interval $[-1,1]$ with density at most $\phi$, find a PNE.%pure NE of the game. 
\medskip

Since the real-valued input to the smoothed $k$-\nashcoord problem is stochastic, the running time of the algorithm that solves it will be stochastic, and the guarantees will be stated either $w.h.p.$ or in expectation (Definition \ref{def:Smooth}). 
%In this paper, we mostly analyze the performance of BRA on smoothed instances of $k$-\nashcoord.
%Our first result shows quasi-polynomial complexity for the BRA. %BRA converges in quasi-polynomial time with high probability. % for smoothed instances

The proof of smoothed-poly running time falls within a framework which has been used in the past to show smoothed-polynomial running time for the FLIP algorithm in local-max-cut~\cite{ER14,A+17,BCC18}, and can also be applied to other local-improvement potential-descent algorithms. This section begins with an overview of this common framework, then proceeds to explain how the required bounds may be shown in our setting. 

\subsection{A Common Framework for Local-Improvement Algorithms}\label{sec:common}

To highlight the framework common to our problem and local-max-cut, we observe that in both cases, the potential function for $k$-\nashcoord, as given in~\eqref{eq:pot}, is an integer linear combination of the payoff values.
In the case of our problem and local-max-cut, it is a 0--1 combination.
The framework can be applied whenever this holds, as long as the potential function's range is also polynomially bounded.
It hinges on the following lemma:

\begin{lem}[{\color{red}\bf Give an Older Citation}]\label{lem:main-praobability} Let $X\in \R^d$ be a vector of $d$ independent random variables where each $X_i$ has density bounded by $\phi$. Let $\alpha_1,\,\dotsc,\,\alpha_r$ be $r$ linearly independent vectors in $\mathbb{Z}^d$.
then the joint density of $(\ip{\alpha_i,X})_{i\in [r]}$ is bounded by $\phi^r$, and for any given $b_1,b_2,\dotsc \in \mathbb{R}$ and $\epsilon>0$, %In particular, if sets $J_i\subset \mathbb{R}$ have measure $\epsilon$, then
\begin{equation}\label{eq:prob-bound-intro}
\Pr\Big[\textstyle\bigwedge_{i=1}^r\ip{\alpha_i,X}\in [b_i,b_i+\epsilon]\Big] \leq (\phi\epsilon)^r
\end{equation}
\end{lem}

Here, the $X$ vector denotes the random input values to the smoothed problem, and the $\alpha$ vectors represent some combination of changes in the potential function. 
Formally, given a potential function $\Phi(\bm  \sigma)$ for some problem, and letting $\bm \sigma_1,\bm \sigma_2,\bm \sigma_3,\dotsc$ be the walk through the state space given by some local-improvement algorithm,
then we have vectors $\alpha_i$ such that $\ip{\alpha_i,X}=\Phi(\bm \sigma_i)-\Phi(\bm \sigma_{i-1})$ for all $i$.
Setting $b_i=0$, the above lemma bounds the probability that {\em every} step of the local-improvement algorithm be a small improvement \mbox{($\ip{\alpha,X}<\epsilon$)}, while still being an improvement \mbox{($\ip{\alpha,X}>0$)}.

Let $\mathcal E$ be the event in the probability statement, that is, $\textstyle\bigwedge_{i=1}^r\ip{\alpha_i,X}\in [0,0+\epsilon]$.
If $\mathcal E$ does not hold, and the sequence is indeed an improving one, then at least one of the improvements must be at least $\epsilon$. If $\mathcal E$ does not hold for {\em any} sequence of $\Omega(n)$ moves, then we can bound the running time of the iterative algorithm by
\[
	\frac n \epsilon\cdot \left(\max_{\sigma} \Phi(\bm \sigma) - \min_{\sigma}\Phi(\bm \sigma)\right)
\]
Finally, if $\Phi$ is bounded in a (quasi)polynomially-sized range, and $\epsilon$ is taken to be $1/(quasi)poly(n)$, then we conclude that the procedure runs in (quasi)polynomial time.

\paragraph{Rank Bound vs Union Bound.} Note that in order to get (quasi)polynomial running time with high probability, first we need to upper bound the probability of event $\mathcal E$. This in turn requires proving a ``high'' rank $r$ on matrix $[\alpha_i]_{i=1}^r$. Furthermore, 
%
%\paragraph{Union Bound.} We must be careful, though: 
for $\mathcal E$ to not occur on {\em any} sequence of $\Omega(n)$ local-improvement moves, we must take the union bound over all sequences of length $\Theta(n)$. It remains then to choose $\epsilon$ correctly to counteract the union bound, for the best rank $r$ which can be shown in general.

This highlights the main technical challenge when applying the common framework: labelling the moves. 
If a move's label is too descriptive --- {\em e.g.} if it contains a state vector --- then the union bound will be much too large. However, if a move's label is too vague --- {\em e.g.} defining a move in $k$-\nashcoord by the player who is moving, but not the strategy they are moving to --- then the rank bound will not be large enough.  
We introduce, in the next section, those parameters which work in our setting.
{\color{red}\bf decide if we need the following} At a high-level our analysis builds on \cite{}. However, handling the game framework where players have multiple strategies throws significant challenges. To keep the exposition relatable to previous approaches we try to use similar notations and terminology as far as possible. 

\subsection{Notation}
Recall the problem of $k$-\nashcoord defined above, and the better-response algorithm (BRA) discussed in Section \ref{}.
We represent each better-response (BR) move by a player-strategy pair $(u,i)$, denoting that player $u$ is replacing strategy $\sigma_u$ by $i$, (assuming $i\neq \sigma_u$). 
We also denote as $\sss^t$ the strategy profile after the $t$\ts{th} BR move. 
Formally, $\sss^0$ is the initial strategy profile, 
and if the move at time $t$ is given by $(u_t,i_t)$, then
\(
	\sss^{t} := (i_t,\sss^{t-1}_{-u_t}).
\)
The change in the potential function at this step is then given by $\payoff(\sss^t) - \payoff(\sss^{t-1})$, which is clearly an integer linear combination of the $A_{uv}(i,j)$ payoff values. 
Since the combinations have integer coefficients, and the payoff values have density bounded by $\phi$, then the total improvement (a random variable) has density at most $\phi$ as well.
For any fixed BR sequence $S$ of length $2nk$, we define these linear combinations as the set of vectors 
$\Lcal=\{L_1,\,L_2,\,\dotsc\}$, where $L_t\in \{-1,0,1\}^{(|E|\times k^2)},\forall t\in [2nk]$, with entries indexed by each of the payoff values. 
The values of its entries are chosen as follows:
\begin{equation*}
L_t((u,i),(v,j))=\left\{\begin{array}{llll}
1 & \text{if: ~~}u_t\in \{u,v\}&\text{and ~~}\sigma^t_u=i&\text{and ~~}\sigma^t_v=j.\\
-1 & \text{if: ~~}u_t\in \{u,v\}&\text{and ~~}\sigma^{t-1}_u=i&\text{and ~~}\sigma^{t-1}_v=j.\\
0 & \text{otherwise.} 
\end{array} \right.
\end{equation*}
That is, every entry signifies whether the corresponding payoff value gets added, removed, or remains unchanged, 
from the potential function. 
The inner product $\ip{L_t,A}$ gives the change in the total payoff of the player who makes a move at time $t$, and thus, the increase in potential due to the $t$\ts{th} move.  

Each of the inner products $\ip{L_t,A}$ can be shown to be unlikely to take values in the range $(0,\epsilon]$ by the assumption of bounded density. To argue that $\Lcal$ has high rank, we partition all players who make a move in the sequence into two sets: 
those players who never play the same strategy twice throughout the whole sequence (non-repeating players), and those players who do (repeating players). 
We will denote these quantities as $p_1$ and $p_2$ respectively, and define $p=p_1+p_2$.
Furthermore, since we will sometimes have to refer to players, and other times to moves, 
we denote as $d$ the number of distinct (player,strategy) pairs which appear in the sequence, and let $q$ denote the number of those moves which are ``return moves,'' that is, moves where a player returns to their original strategy.
Note that for any sequence of moves $S$, we have $p(S)\leq d(S)\leq k\cdot p(S)$.
{\color{red}\bf Is $q$ the same things as $p_2$??} \rnote{No! But it seems we should be able to merge these two, no? Like if we define notation to count repeat (player,strategy) pairs starting with $\sigma^0$?}

\subsection{Critical Blocks and Small Union Bounds}\label{sec:union-critical}
The notion of {\em critical block}, introduced in \cite{A+17}, allows us to translate rank and union bounds in terms of $p$ and $d$ values, into bounds which are linear in the sequence size.
Formally, let $\ell(S)$ be the length of the sequence, and call a sequence $S$ ``diverse'' if $\ell(S)< 2(d(S)-q(S))$. 
A sequence is diverse if, for its size, it has many different moves. 
A {\em critical block} is a contiguous sub-sequence which is, in some sense, maximally diverse. 
That is, a block $B\subseteq S$ such that $\ell(B)\geq 2(d(S)-q(S))$, and for every $B'\subseteq B$, $B's$ is diverse.
To see that such a block must exist, note that any sequence of length 1 must be diverse, and any sequence of length $2nk$ can not be diverse. Therefore, if we begin with a sequence of length $2nk$, it must contain a ``maximally diverse'' subsequence.

It then becomes clear that, restricting our attention to critical blocks will allow us to show $\Theta(\ell)$ bounds by instead showing $\Theta(p)$ bounds, if we take $k$ to be a constant.
However, these critical blocks might be significantly smaller than the original $2nk$-sized sequence, which introduces some difficulties for the union bound.  

Now, recall that we must consider {\em any} sequence of $\ell$ player-strategy pairs. This na\"ively have $k^n$ possible initial strategy configurations, and $(nk)^\ell$ choices for the $\ell$ moves, and so we have a union bound of size $k^n (nk)^\ell$.
If we can show a rank lower-bound of $r$, then we get success probability
\[
	1-k^n (nk)^\ell (\phi\epsilon)^{r}
\]
Note that we must have $r\leq \ell$, since $\ell$ is the number of columns whose rank we are bounding.
If we had $r\geq \Omega(n)$, then to get 
polynomially decaying probability of failure, we can set $1/\epsilon = \phi(nk)^{O(k)}$, 
which gives an overall run-time of $(nk\phi)^{O(k)}$. 
This runtime does indeed match the results that we prove for the case of complete game graphs.
However, when $\ell$, and subsequently $r$, are much smaller than $n$, then the $k^n$ term dominates the probability bound, and $\epsilon$ is needed to be significantly smaller.

Observe that the $k^n$ term is the effect of the initial configuration of those players which do not move in the sequence, but do have an effect on the potential function. 
There are two possible options for getting around this issue.
The one, introduced in~\cite{A+17}, isolates the effect of these players, and ``buckets'' their influence.
Thus, we need not keep track of each player's state, but instead, of the value of their contributions.
The other, introduced in~\cite{ER14}, and extended in~\cite{BCC18}, uses the notion of a ``cyclic sum,'' which altogether eliminates the effect of non-moving (or {\em inactive}) players' strategy from the linear combinations. 
It does, however, change the vectors being considered, and makes the analysis more subtle.

\paragraph{Union Bounds via Bucketing.}
Note, the potential, $\sum_{uv\in E}A_{uv}(\sigma_u,\sigma_v)$ can be separated into terms between two players present in the sequence ({\em active}), which we can na\"ively union-bound, terms between two inactive players, which remain constant, and terms between an active and an inactive player. This latter value can be split up into different sums for each active player, of their payoffs with inactive players.
These values can then be rounded to the nearest multiple of $\epsilon$, and instead of recording the states of the non-moving players, we just record which of the $2n\epsilon$ possible values it has been rounded to, and take the additive error into account when considering the probability bound. 
This leaves a union bound of the form $k^p (n/\epsilon)^d$, one term for each of the distinct moves of the active players.
Some shifting of the weight of the initial strategies of the active players into the constant term allows us to instead get a bound of the form $k^p (n/\epsilon)^{d-q} (nk)^\ell$.
These exponents are more promising than the $k^n$ term of the na\"ive bound. However, note that the negative exponent on the $\epsilon$ term requires the rank bound to at least match it. 
We will later see how a rank bound of the form $r\geq d-q+\Omega(p_1)$ can be shown, which allows the probability bound to look more like $k^p (nk)^{kp} (\phi\epsilon)^p$, as desired.

\paragraph{Union Bounds via Cyclic Sums}
This union bound is not for the number of possible sequences of the $L$ vectors as above, but instead, is simply the na\"ive bound on a difference set of vectors, which allow us to show similar results. 
These vectors are sums of a subset of the $L$ vectors, and are only defined when {\em repeat moves} are made.
That is, either repeat occurrences of the same (player,strategy) pair, or a return move.
These sums allow us to cancel out the effect of inactive players.
Let $L_t$ be the $t$-th column of $L$, and suppose player $u$ moved to strategy $i$ twice. 
Let $\tau_0$ be the first occurrence of $(u,i)$ in the BR sequence, and let $\tau_1,\tau_2,\dotsc,\tau_k$ be all subsequent appearances of $u$ in the sequence, playing any strategy. Suppose $\tau_m$ is the second occurrence of $(u,i)$ in the BR sequence. 
Let player $v$ be some player who starts in strategy $j$, and never deviates.
Then the sum $L_{\tau_1}+L_{\tau_2}+\dotsm+L_{\tau_m}$ cancels out all $(uv,\cdot,\cdot)$ entries, since each one gets added in one column, and removed from the next (cyclically). These cyclical sums, therefore, do not depend on the initial configurations of the players who do not appear in the sequence.

Thus, taking these summed vectors, we need not consider the initial configurations of the inactive players, and can take a union bound of the form $O(k^\ell(nk)^\ell)$. 
However, it does affect the probability computation a bit: to bound the probability that $\ip{L_t,A}$ lie in $(0,\epsilon)$ for all $t$, it suffices to bound the probability that $\ip{L_{\tau_1}+L_{\tau_2}+\dotsm+L_{\tau_m},\,A}$ lie in $(0,n\epsilon)$. 

It remains to show how the above rank bounds can be attained, and conclude that the BRA terminates in polynomial time with high probability, and in expectation.

\subsection{Smoothed Polynomial Complexity of the BRA} \label{sec:complete-graph-rank}
We wish to show, for the two above union bounds to be useful, a bound of the form $r\geq d(S)-q(S)+\Omega(p_1(S))$ on the usual $L$ vectors, and a bound of the form $r\geq \Omega(p_2(S))$ for the cyclic-sum vectors.
The ``common framework'' of section~\ref{sec:common} allows us then to show.

\begin{thm}\label{thm:poly}
Given a smoothed instance of {\em $k$-\nashcoord} on a complete game graph, and with an arbitrary initial strategy profile, 
then any execution of BRA where improvements are chosen arbitrarily will converge to a PNE in at most 
% $(nk\phi)^{O(k+\eta)}$ steps, 
% with probability \mbox{$1-1/(nk\phi)^{O(\eta)}$}, for any fixed $\eta>0$.
$(nk\phi)^{O(k)}$ steps, with probability \mbox{$1-1/poly(n,k,\phi)$}.
\end{thm}
\vspace*{-1ex}

We note that the probability value in the above statement is over the possible choices of payoff values for the Network game, and not over executions of the BR algorithm. This statement holds true regardless of how BRA is implemented, even adversarially.
By complete game graph, we simply mean that all payoff values are random variables, and any two players must participate in some ``edge game.'' We can not simply take missing edges to be 0-payoff games, as that would not be perturbed.
This fits the model of most known smoothed polynomial-time algorithms ($e.g.$ \cite{ST04,SST06,ERV14,A+17,BCC18}) which do require {\em every} parameter to be perturbed. 
We will later discuss results in the incomplete-graph cases, where missing edges are assumed to be 0-payoff games, unperturbed.

We also present a meta-theorem which abstracts a pre-existing result,
and state that for any problem in PLS with bounded total improvement, a $w.h.p.$ smoothed complexity bound implies an expected time bound (see Section \ref{sec:exp}). 
This, together with theorem \ref{thm:poly}, implies

\begin{thm}\label{thm:poly-expectation}
Given a smoothed instance of {\em $k$-\nashcoord} with an arbitrary initial strategy profile, 
then any execution of BRA where improvements are chosen arbitrarily will converge to a PNE in at most $(nk\phi)^{O(k)}$ steps in expectation, for a complete game graph.
\end{thm}

Thus it remains to show the two rank bounds described above. 
Our rank bounds will be shown by identifying sufficiently large upper-triangular submatrices of $\mathcal L$.
As discussed in section~\ref{sec:common}, the bounds shown are sensitive to the column labels, since we may only use these when talking about worst-case $\mathcal L$ matrices. In fact, we will see that the $d-q+\Omega(p_1)$ bound can not be raised to a $d+\Omega(p_1)$ bound, which is why it was essential to get the ``bucketing'' union bound to need only $d-q$ terms.

\paragraph{Rank Bounds on $\mathcal L$.}
If there are no inactive players, then as proved in Lemma \ref{lem:all-active}, it is easy to argue a minimum rank of $n-1$ for vectors of $\Lcal$ and pair it with the na\"ive union bound. Thus, we restrict our attention to the case where there are many inactive players.

To bound the rank, we first divide the sequence into blocks, 
where the endpoints of each block are the {\em last} occurrence of a non-repeating player in the BR sequence. 
(The blocks do not include these players' final moves). 
These blocks are termed \textit{transition blocks}, and the vectors inside and outside the transition block can be ``separated,'' by whether they contain a non-zero values on the associated payoff entries.
Let $v$ be the non-repeating player who appears for the last time, and let $j$ be her final strategy.
Let $u$ be some other player, then vectors inside the transition blocks will have 0 coefficient for the $(uv,*,j)$ term, while the vectors outside will have non-zero.

Let $T$ be some transition block, then it can be shown that the rank of the moves of $T$ is at least $d(T)-q(T)$.
Recall that we are restricting ourselves to some critical block $B$: this implies that the rank of the transition blocks is at least half their length, since $T\subsetneq B$, and there $\ell(T)< 2(d(T)-q(T))$, by criticality. 
We can also show that the final moves of the non-repeating players are themselves independent of all other columns, which adds a factor $p_1$ to the rank. This, and the transition-block observation, gives us our desired bounds.

\paragraph{Rank Bounds on cyclic sums.}
{\em\color{red} This kinda depends on how the proof goes..... I'll write what I guess to be the correct form, but it needs double-checking for sure.}
This rank bound will be applicable in the case of non-complete graphs as well as complete.
Recall, from section~\ref{sec:union-crit}, the notion of the ``cyclic sum'' vector, the sum of all moves of some repeating player between two instances of the same move, excluding the first, including the last.
Clearly, this sum must form a non-zero vector, as otherwise, the sequence is returning to the same state as the original time the move was played, which makes it non-improving. 
This allows us to form an auxiliary digraph, where the nodes are the active players.
Create an edge from a repeating player $u$ to any other player $v$, if {\em some} cyclic sum for $u$ contains a non-zero entry with $v$. 
We show that there exists a way to bi-partition the nodes of this graph such that for one of the two partitions, 1. it contains at least half of the repeating players, and 2. each node in this partition has an out-neighbour outside of the partition. 
These edges, and their associated matrix entries, allow us to form an upper-triangular submatrix of rank $\Omega(p_2)$, on the set of cyclic sums.








\subsection{Smoothed Quasipolynomial Complexity of the BRA on General Graphs}
We have shown, above, that for complete game graphs, the BRA terminates in polynomial time with high probability, and as discussed, in expectation.
We discuss here how the cyclic-sum interpretation immediately gives quasi-polynomial smoothed complexity for arbitrary game graphs (Theorem~\ref{thm:qpoly}), based on a {\color{red}\bf a lemma of~\cite{ER14}}. 
This lemma states that any sequence of $\Omega(n)$ {\em improving} moves must have at least $\Omega(n/\log n)$ distinct repeated moves. 
Therefore, a sequence of $\Omega(nk)$ player-strategy pairs in a BRA sequence must contain at least $\Omega(nk/\log(nk))$ distinct recurring pairs, and therefore, $p_2\geq \Omega(n/\log(nk))$, since each player can only appear in $k$ distinct pairs. 
This fact, combined with the discussion from section~\ref{sec:complete-graph-rank}, allows us to show the following:
\begin{thm}\label{thm:qpoly}
Given a smoothed instance of {\em $k$-\nashcoord} with an arbitrary initial strategy profile, 
then any execution of a BR algorithm where improvements are chosen arbitrarily will converge to a PNE in at most 
% $O(\phi(nk)^{(1+\eta)k\log(nk)})$
$\phi\cdot (nk)^{O(k\log(nk))}$
% steps, with probability $1-1/(nk)^{O(\eta)}$, for any fixed $\eta>0$.
steps, with probability $1-1/poly(n,k)$.
\end{thm}
\vspace*{-1ex}

Along with the same meta-theorem that was used to show polynomial expected-time convergence of the BRA for complete graphs, we also show

\begin{thm}\label{thm:poly-expectation}
Given a smoothed instance of {\em $k$-\nashcoord} with an arbitrary initial strategy profile, 
then any execution of BRA where improvements are chosen arbitrarily will converge to a PNE in at most 
$O(\phi)\cdot (nk)^{O(k\log(nk))}$ steps in expectation.
\end{thm}



















\subsection{Smoothness-Preserving Reduction to 1- and 2-\maxcut}\label{sec:overview-reduction}
We have shown, above, that the BRA converges quickly for $k$-\nashcoord. 
Our second set of results analyzes {\em smoothness-preserving} reductions for the $k$-\nashcoord problem, to give alternate algorithms, and to introduce a reduction framework for smoothed problems.
The authors of this paper have not found any prior notion of smoothness-preserving reduction.

Recall the {\em smoothness-preserving} reductions defined in Section \ref{sec:PrelSmooth}. In this section, we discuss a  result explaining how these reduciton notions may be applied (Theorem \ref{thm:meta-red}), and then give an overview of how to obtain such reductions for the $k$-\nashcoord problem and prove Theorems \ref{thm:2strat} and \ref{thm:kstrat} below.
All the details and proofs are in Section \ref{sec:red}.

First, if problem $\CP$ admits a {\em strong} smoothness-preserving reduction to problem $\CQ$, and $\CQ$ has smoothed polynomial algorithm in terms of {\em whp}, then so does $\CP$. Since such reductions allow use of extra randomness, we need to ensure that it does not affect the {\em high-probability} statement by much. We do this using the Markov's inequality and careful interpretation of the extra randomness. 

Second, if problem $\CP$ admits a {\em weak} smoothness-preserving reduction to the {\em local-max-cut} with (arbitrary) complete graphs, then $\CP$ has smoothed (quasi-polynomial) polynomial complexity. Here, the analysis builds on the first result, but also crucially depends on the rank-based analysis of \cite{ER14} and \cite{A+17} for the local-max-cut.
These are formalized in the following result: 
\begin{thm}\label{thm:meta-red}
Suppose problem $\CQ$ has (quasi-)polynomial smoothed complexity. Then, if problem $\CP$ admits a strong smoothness-preserving reduction to $\CQ$, then $\CP$ also has (quasi-)polynomial smoothed complexity. If instead, $\CP$ admits a weak smoothness-preserving reduction to local-max-cut on an (arbitrary) complete graph, then $\CP$ again has a (quasi)polynomial smoothed complexity.
%If instead, $\CP$ admits a weak smoothness-preserving reduction to local-max-cut with (in)complete graph, then $\CP$ has a (quasi)polynomial smoothed complexity.
\end{thm}
\vspace*{-1ex}

 %FLIP algorithm for the local-max-cut is based on viewing every step as linear-combination of the input parameters, and the rank argument for these linear-combinations. 
%The proofs of \cite{ER14} and \cite{A+17} mainly show that linear combinations of the edge weights have high rank, and then directly apply Lemma~\ref{lem:praobability} to show that the improvement happens with high probability. Let $M$ be a full rank $d\times d$ matrix, and note that $\ip{\alpha,MX} = \ip{M^{\mathsf T}\alpha, X}$. We conclude then that the input to Local Max Cut need not be independent random variables with bounded density. Instead, it suffices to have the edge weights be full-rank, integer linear combinations of a random variable with bounded density, since we need $M^{\mathsf T}\alpha$ to be an integer vector for all integer $\alpha$. Therefore, a {\em weak} smoothness-preserving reduction to Local Max Cut on an (in)complete graph suffices to show smoothed (quasi-)polynomial complexity.
\medskip

This allows us to extend smoothed efficient algorithm from one problem to another. 
Ideally we would like to show {\em strong} reductions. However, we manage to show {\em weak} reductions from $k$-\nashcoord to $1$- or $2$-\maxcut. %$(i)$ from $2$-\nashcoord to $1$-\maxcut (local-max-cut), and $(ii)$ from $k$-\nashcoord to $2$-\maxcut. 
Note that, smoothed complexity of $2$-\maxcut is not known yet, but we believe that $2$-FLIP algorithm may admit a similar rank-based analysis as FLIP. And that will give a smoothed efficient algorithm for $k$-\nashcoord with arbitrary $k$. %Next, we discuss the second reduction.


%\begin{comment}
%Whereas in the previous section we directly showed that the $k$-\nashcoord problem can be solved in polynomial time with high probability for fixed $k$,
%we define here a notion of {\em smoothness-preserving} reduction between search problems, 
%which allows us to reduce this problem to $1$- or $2$-\maxcut. 
%This latter problem is not known to have (quasi)polynomial smoothed complexity, but if it were, this reduction would imply (quasi)polynomial smoothed complexity for $k$-\nashcoord with variable $k$.
%
%Recall from Section~\ref{sec:PrelSmooth} the notions of Strong and Weak Smoothness Preserving Reduction. 
%% Given search problems with discrete inputs and real-value parameters ($e.g.$ a Network Game with its payoff values, or a graph with edge weights) 
%% we want to convert from instances of one problem to instances of the other, such that solutions to the latter may be lifted to solutions of the former.
%% However, we insist that the conversion is done in such a way that when the parameters of the problem being reduced are independent random variables, , but in such a way that any independence over the parameters of the former 
%we wish to show that $k$-\nashcoord admits a weak smoothness-preserving reduction to $2$-\maxcut.
%The proofs of \cite{ER14} and \cite{A+17} mainly show that linear combinations of the edge weights have high rank, and then directly apply Lemma~\ref{lem:praobability} to show that the improvement happens with high probability. 
%Let $M$ be a full rank $d\times d$ matrix, and note that $\ip{\alpha,MX} = \ip{M^{\mathsf T}\alpha, X}$.
%We conclude then that the input to local-max-cut need not be independent random variables with bounded density.
%Instead, it suffices to have the edge weights be full-rank, integer linear combinations of a random variable with bounded density, since we need $M^{\mathsf T}\alpha$ to be an integer vector for all integer $\alpha$.
%Therefore, a {\em weak} smoothness-preserving reduction to local-max-cut on an (in)complete graph suffices to show smoothed (quasi-)polynomial complexity.
%\end{comment}

\paragraph{$k$-\nashcoord to $2$-\maxcut.}
We wish to show the following result:
\begin{thm}\label{thm:kstrat}
% There exists a {\em weak smoothness-preserving} reduction from k-\nashcoord to {\em 2-\maxcut}.
$k$-\nashcoord admits a {\em weak} smoothness-preserving reduction to 2-\maxcut.
\end{thm}
\vspace*{-1ex}

Though this result does not immediately provide an algorithm to solve $k$-\nashcoord, we show that it does raise the following implication:
If we can show that the 2-FLIP algorithm solves smoothed instances of \mbox{2-\maxcut} in (quasi-)polynomial time through rank-based analysis similar to FLIP, then \nashcoord has (quasi-)polynomial smoothed complexity for $k$ in the input, rather than fixed $k$.
We leave the smoothed analysis of 2-\maxcut as an open problem.

The idea for the reduction is, given an instance of a Network Coordination Game, construct a graph whose locally optimal cuts can be mapped to strategy profiles, and the total cut value of said cuts is equal to the total payoff of the associated strategy profile.
To do this, we construct a graph with $nk+2$ nodes, two terminals $s$ and $t$, and $nk$ nodes indexed by player-strategy pairs $(u,i)$. 
Nodes $s$ and $t$ are connected to every other node in the graph, and for each player $u$ and strategy $i$, there is an edge from node $(u,i)$ to node $(u,j)$ for all $j\neq i$.
Furthermore, if player $u$ and $v$ share an edge in the game graph ($i.e.$ play together), there is also an edge from $(u,i)$ to $(v,j)$ for all $1\leq i,j\leq k$.
Therefore, the cut graph is complete if and only if the game graph is.
Call a cut $S,T$ valid if it is an $s$-$t$ cut with $s\in S$ and $t\in T$, and if $S$ contains at most one node $(u,i)$ for each player $u$.
Now, for any valid $s$-$t$ cut, we can interpret this cut as determining a strategy profile as follows:
If player $u$ appears in $S$ the cut paired with strategy $i$, then set $\sigma_u=i$. 
Otherwise, set $\sigma_u=0$, a ``dummy'' strategy with bad payoff. Call this profile $\sss(S)$.
We wish to choose edge weights such that all locally maximal cuts are valid cuts, 
and also such that for any valid cut $S$, the total cut value is equal to $\payoff(\sss(S))$.

To show that this reduction is indeed a smoothness-preserving reduction, it suffices to show that $\sss(S)$ is a PNE if and only if $S$ is a local-max-cut up to 2 flips, and that for random payoffs with bounded density, the edge weights in the reduction also have bounded density, and are full-rank combinations of independent random variables.
This last condition is guaranteed by choosing the edge weights as a full-rank, integer, linear combination of the payoff values.
It remains to show that this is possible while ensuring the first condition.
Indeed, we ensure that any non-valid cut can always be improved by flipping at least one node.
Furthermore, we ensure that any valid cut has total cut value equal to the total payoff of the associated strategy profile.
Since replacing $\sigma_u$ with $\sigma'_u$ is equivalent to dropping $(u,\sigma_u)$ from the cut and adding $(u,\sigma'_u)$, then any locally optimal cut up to two flips must be equivalent to a Nash Equilibrium.
Thus, we achieve a weak reduction, proving Theorem \ref{thm:kstrat}. %achieve a weak reduction. 

\paragraph{\bf $2$-\nashcoord to $1$-\maxcut.} Here, we take a slightly different reduction, where there are $n+2$ nodes in the graph, and any $s$-$t$ cut is interpreted as follows: if $u$ is on the same side as $s$ of the cut, $\sigma_u=1$, otherwise, $\sigma_u=2$. The same analysis goes through, but now, locally max cuts up to one flip are Nash Equilibria, which provides a weak smoothness-preserving reduction from 2-\nashcoord to 1-\maxcut, showing the following result:
\begin{thm}\label{thm:2strat}
% There exists a {\em weak} smoothness-preserving reduction from 2-\nashcoord to $1$-\maxcut. 
2-\nashcoord admits a {\em weak} smoothness-preserving reduction to 1-\maxcut.
\end{thm}
\vspace*{-1ex}
The FLIP algorithm for $1$-\maxcut has smoothed quasi-polynomial running time in general \cite{ER14}, and smoothed polynomial running time if $G$ is a complete graph \cite{A+17}. A recent result \cite{BCC18} seems to have improved the running time of the latter, and so this reduction allows us to provide better bounds on the performance of BRA in the case $k=2$. These local-max-cut results, together with Theorems \ref{thm:meta-red} and \ref{thm:2strat}, give an alternate smoothed efficient algorithm for the $2$-\nashcoord problem.


==> Section-CG-Quasipoly-congestion.tex <==

In this section, we define the notion of {\em $(k,\ell)$-congestion games}, and show that the same sequential-improvement BR algorithm also has smoothed quasi-polynomial time complexity in this model, for constant $k$ and $\ell$. It is worth noting that this model of congestion game generalizes network coordination games, which can be shown are $(k,2)$-congestion games, and local max cut, which can be shown to be a $(2,2)$-congestion game. In fact, the results in this section naturally generalize past results.

\subsection{Notation}

\begin{defn}
A \textit{congestion game} among $n$ players is defined by a set of resources $E$ of size $r$, an explicitly described strategy set $S_i\subseteq 2^E$ for all players$i\in [n]$, and for each resource $e\in E$, a monotone cost vector $c_e\in\mathbb R^{n+1}$, where we assume $c_e(i)-c_e(i-1)\in [0,1]$ for all $i\geq 1$. 
A strategy profile $\sss=(s_1,\,s_2,\,\dotsc,\,s_{n-1},\,s_n\}$, with $s_i\in S_i$ for all $i\in [n]$ denotes a particular outcome of the game. Let $n_e(\sss)$ denote the number of strategies $s_i$ in $\sss$ which include resource $e$, {\em i.e.} $n_e:=|\{i\in[n] : e\in s_i\}|$, then the cost of resource $e$ at profile $\sss$ is $c_e(n_e(\sss))$. 
Thus, the cost player $i$ pays is $\sum_{e\in s_i} c_e(n_e(\sss))$.
\end{defn} 

The objective is to find a {\em Nash equilibrium} of these games, which is defined naturally. We include the formal definition below for completeness.

\begin{defn}
A \textit{Nash equilibrium} of a congestion game is a strategy profile whose cost cannot be decreased by unilateral deviation of any player. Formally, 
\[
	\sum_{e\in s_i} c_e(n_e(s_i,\sss_{-i})) \leq \sum_{e\in s_i'} c_e(n_e(s_i',\sss_{-i}))\quad
    \text{ ~ for all ~ }i\in [n]\text{ ~ and ~ }s_i'\in S_i
\]
% $$c(s)\ge c(s_{i}',s_{-i}),\forall i\in [n], s_{i}'\neq s_i.$$ 
$(s_{i}',\sss_{-i})$ denotes a strategy profile where every player except $i$ chooses the same strategy as in~$\sss$.
\end{defn}

In fact, similarly to the network coordination games, this game also admits a {\em potential function} 
\begin{equation}
	\Phi(\sss):= \textstyle\sum_{e\in E}\sum_{i=0}^{n_e(\sss)} c_e(i)
\end{equation}
It can be shown that $\sss$ is a Nash equilibrium if for any player $i$ and strategy $s_i\in S_i$, $\Phi(s_i,\sss_{-i})\leq \Phi(s_i',\sss_{-i})$. 
In fact, if $\psi_i(\sss)$ is the cost payed by player $i$ at profile $\sss$, then 
\[\psi_i(s_i,\sss_{-i}) - \psi_i(s_i',\sss_{-i}) = \Phi_i(s_i,\sss_{-i}) - \Phi_i(s_i',\sss_{-i})\]
This observation, and others, may be found at~\cite{RoughLectureCongestion}

If two strategy profiles are said to be as {\em adjacent} when they differ in the strategy choice of a single player, then a PNE of a congestion game is a profile which minimizes $\Phi$ in its neighbourhood. To find a local optimum of $\Phi$, the better-response algorithm (BRA) for the game starts at an arbitrary strategy profile $\sss^0$, and recursively checks if the total cost can be improved by unilateral deviation of some player, and moves to an arbitrary profile with non zero improvement. That is, for all $t\geq 0$, if $\sss$ is adjacent to $\sss^t$ with $\Phi(\sss)>\Phi(\sss^t)$, then set $\sss^{t+1}\gets \sss$. This process continues until we reach a PNE of the game.

Although the aim of a congestion game is to (locally) \textit{minimize} the total cost, to use the technical lemmas of $k$-\nashcoord we modify the input by inverting the signs of all entries of the cost vector, and aim to (locally) maximize the potential $-\Phi(\sss)=-\sum_{e\in E}\sum_{i\le n_e(\sss)}c_e(i)$. Hence forth, we abuse notation slightly and assume the given cost vector is this sign inverted-vector.


%We now prove the BRA on a congestion game has smoothed quasi polynomial time complexity.

\subsection{Model}

We define a $(k,\ell)$-congestion game, as a congestion game where the number of distinct strategies a player can choose from is at most $k$ ($|S_i|\leq k$ for all $i$), and any resource belongs in at most $\ell$ strategies overall ($|\{s\in \bigcup_{i=1}^n S_i:e\in s\}|\leq \ell$ for all $e\in E$). We denote the problem of finding a PNE in a $(k,\ell)$-congestion game as $(k,\ell)$-\Congestion.

%We represent the cost functions of the game by a vector $C\in [-1,1]^{r\times (\ell+1)}$, where the $(e,i)^{th}$ entry is $c_e(i)$, i.e. the cost of using resource $e$ if $i$ players are currently using it ($n_e=i$). 

A move in the game is a tuple $(u,s_u)$, denoting that player $u$ deviates to strategy $s_u$. We represent every move by an $r\cdot (\ell+1)$-length vector $L$, where the $(e,i)^{th}$ entry is $+1$ if $n_e$ went from $i\pm 1$ to $i$ due to the move, $-1$ if $n_e$ went $i$ to $i\pm 1$ due to the move, and $0$ if the move leaves $n_e$ unchanged. 
Let $C$ be the $r(\ell+1)$-dimensional vector whose $(e,i)$-th entry is $\sum_{j=1}^i c_e(j)$, for all $e\in E$ and all $0\leq i\leq \ell$.
Note, then, that given a move vector $L_t$, the inner product $\ip{L_t,C}=\Phi(\sss^t)-\Phi(\sss^{t-1})$. 

Recall, from section~\ref{sec:notation}, the definitions of \Lset ($\Lcal$), {\em active} and {\em inactive} players, and {\em repeating} and {\em non-repeating} players, whose quantities are denoted as $p_2$ and $p_1$, respectively. A sequence of BR moves thus generates a \Lset as before, $\Lcal=\{L_1,L_2,..\}$, where $L_t$ is defined just above.

The main difference between this model and that of $k$-\nashcoord is that, instead of the rows of the vectors being denotes by pairs of moves (``$((u,i)(v,j))$''), they are denoted by resource-utilization amounts, (``$(e,i)$''). In most other regards, the matrix arguments are similar.
% This model is different from the model of $k$-\nashcoord. The entries of a move in $k$-\nashcoord are $2$-tuples moves. An entry $((u,i),(v,j))$ is non zero in a particular move vector $L_t$ if players $u$ and $v$ deviate from or to strategies $i$ and $j$ respectively, \textit{and one of the two is playing at time instant $t$}. Hence, the set of non zero entries in every move can be restricted to a particular subset of entries (only the tuples containing the current move).

% In $k,\ell$-\Congestion, move vector entries do not directly correspond to strategies or moves of players, rather they depend on the set of resources from which player strategies are formed. As strategy sets of players are not same in general, but the universe of resources from which the strategy sets arise is consistent among all players, the rows must be defined based on these. However, now one cannot find such a strict subset of entries that can be non zero.  

%However, modeling the BR sequence by tracking the number of players using a particular resource, now allows non zero entries in move vectors for any 

\paragraph{Smoothed $(k,\ell)$-congestion games.}
To analyze the smoothed complexity of this problem, we must define a smoothed model of congestion games. 
Since the real-valued input to the problem is the cost vectors of resource utilization, the random input must be the cost vectors. However, we have required $c_e(i)$ to be monotone in $i$. 
To this end, define the differential cost $d_e(i) := c_e(i)-c_e(i-1)$, with $d_e(0):= c_e(0)$. Then, we may restrict $d_e(i)$ to be a random variable supported on $[0,1]$ with density at most $\phi$, and then the cost function $c_e(i) = \sum_{j=0}^i d_e(i)$ will be monotone. However, the $C$ vector neither consists of the $c_e$ values or the $d_e$ values. 
Instead, let $\bar c_e(i) = \sum_{j=0}^i c_e(i) = \sum_{j=0}^i \sum_{m=0}^j d_e(m)$. 
Note, however, that the $c_e$'s are a full-rank combination of the $d_e$'s, and the $\bar c_e$'s are a full-rank combination of the $c_e$'s, and so there must exist a square, full-rank matrix $U$ such that $C= UD$, where $D$ is the vector of $d_e$ values.

An instance of a {\em smoothed $(k,\ell)$-congestion game} is then given by a ground set $E$, $n$ sets of strategies $S_i\subseteq 2^E$, and a random vector $D$ of differential payoff values. We wish to show:

% Note that cost functions for any resource in congestion games are usually monotonically increasing in the number of players using the resource. That is, $c_e(i)\ge c_e(j),\ i\ge j,$ for all resources $e\in E$. Monotonicity in entries cannot be ensured when the cost vector is directly randomly chosen. Instead, we consider the entries of the chosen vector to be $\overline{C}(e,i)=c_e(i)-c_e(i-1)$, for all $i\ge 1$, and $\overline{C}(e,0)=c_e(0)$, for all resources $e\in E$. The marginal increase in cost when $1$ more player uses a particular resource, does not have constraints and can be any value. Hence, all entries of $\overline{C}$ can be chosen randomly.

% It is clear that the cost $c_e(i)$ is related to entries of $\overline{C}$ as $c_e(i)=\sum_{j\le i} \overline{C}(e,j)$. Hence to obtain the cost vector $C$ for the game from the smoothed input, we consider the block-lower-triangular matrix $U$ defined above. The product $C=U\overline{C}$ is the cost vector for the game. 

% [[[[]]]]

% Now, in the network-coordination game result, we required
% We want the inner product to reflect the change in the cost of the game $\phi(\sss^t)-\phi(\sss^{t-1})$ after the move. To allow this, we consider a $2$-dimensional block-lower-triangular matrix $U$ of size $(r\times (\ell+1))^2$, where the entries are defined as $U((e,i),(e',j))=1,\ j\le i, e'=e$, $U((e,i),(e',j))=0$ otherwise. Define the product vector $\Gamma=UC$. $\Gamma(e,i)$ reflects the cumulative cost when at most $i$ players use $e$, that is, $\Gamma(e,i)=\sum_{j\le i} c_e(j)$. The inner product $\ip{L_t,\Gamma}$ then is the change in potential, as 
% $$\ip{L_t,\Gamma}=\sum_e \Gamma(n_e(\sss^t))-\Gamma(n_e(\sss^{t-1}))=\sum_{i\le n_e(\sss^t)}c_e(i)-\sum_{i\le n_e(\sss^{t-1})}c_e(i))=\phi(\sss^t)-\phi(\sss^{t-1}).$$


% [[[[]]]]


\begin{thm}\label{thm:CGquasipoly}
Given a smoothed instance of {\em $(k,\ell)$-\Congestion} with an arbitrary initial strategy profile, 
then any execution of a BR algorithm where improvements are chosen arbitrarily will converge to a PNE in at most 
$\phi r(nk)^{O(\ell k\log(nk))}$ steps, with probability $1-1/poly(n,k)$.
\end{thm}

%The rest of this section will formally prove this theorem. 
The idea is, again, to prove that any arbitrary $O(nk)$-length BR sequence of sufficiently high rank has polynomially large improvement {\em w.h.p.}, then applying a union bound over all choices for a sequence, to prove that the any execution of BRA over a sufficiently long sequence will have good improvement with good probability. This will allow us to prove the above result. We first show:


%\begin{rem}
%In local-max-cut the only variable parameter was $n$, the number of players, (the \textit{strategies} for a player here were the side of the cut), and in $k$-\nashcoord there are two distinct notions, the players ($n$) and strategies ($k$). In $k,\ell$-\Congestion there are three parameters, the players, their strategies, and the resources. 
%\end{rem}

%\Rucha{proof not done yet!}
\begin{lem}\label{lem:rank-p2-congestion}
Let $S$ be a BR sequence in a $(k,\ell)$-congestion game, and let $\Lcal=\{L_1,\,L_2,\,\dotsc\}$ be its \Lset.
Then the span of $\Lcal$ contains at least $p_2(S)/\ell$ linearly independent vectors $V_1,\,\dotsc,\,V_{p_2/\ell}$ that are all 0-1 combinations of the $L_i$'s.
\end{lem}
\begin{proof}
	This proof follows the outline of that of lemma~\ref{lem:rank-p2}.
	Fix a repeating player $u$, and denote one of its repeating strategies as $s_u$. 
    Let $t_u$ be the first occurrence of $(u,s_u)$ in the sequence, setting $t_u=0$ if $i_u=\sss^0_u$.
    Let $t_{u}'$ be the first occurrence of $(u,s_u)$ after $t_u$. 
    Formally, if $S=\{(v_1,s_1),(v_2,s_2),\dotsm\}$, then $v_{t_u}=v_{t'_{u}}=u$, $s_{t_u}=s_{t'_{u}}=s_u$, and $(v_t,s_t)\neq (u,s_u),\ \forall t_u<t<t'_{u}$. Consider the vector $V(u) = \sum_{\tau= t_u}^{t'_u}L_{\tau}$. 
    Vector $V(u)$ is a 0-1 combination of the $L_i's$ by construction. We will show that at least $p_2/\ell$ of these must be linearly independent.
    
    \hrule
    
    Note that, the sum of all move vectors between two consecutive repeating moves of a player is a vector with entry $1$ in a row $(e,j)$ if the number of players using resource $e$ is $j$ at the end of the second appearance of the move, and $-1$ in the row $(e,j+1)$ or $(e,j-1)$, denoting that prior to this move the number of such players was different by $1$. The inner product $\ip{V(u),C}$ represents the total change in the cost of the game because of the sequence of moves between times $t_u$ and $t_{u_r}$. Thus, by definition of an improving sequence, at least one entry in every $V(u)$ must be non zero. 
     
Consider a matrix $M_1$ where the columns are all vectors $V(u)$ defined above, arranged in chronological order of the second occurrence of the repeated move. We rename the players in this matrix by $1,2,\dotsc$ for notational convenience. Every column in $M_1$ must have a $1$ entry. %Let $E_i=\{(e_i,n_i)=1\}$ denote the set of $1$ entries corresponding to player $i$'s vector $V(i)$. 

As a resource $e_i$ can belong in at most $\ell$ strategies at once, it is non zero in at most $\ell$ of the column vectors $V(i)$s. Denote the set of column vectors where $(e_i,n_i)\ne 0$ by $V_{(e_i,n_i)}$. 

We create a matrix $M$ by taking exactly one vector from every group of vectors $V_{(e_i,n_i)}$, and removing the rest from $M_1$. This leaves a set of at least $p_2/\ell$ vectors, that each have at least one non zero ($1$) entry, that is zero in all the rest. Thus, by a suitable rearrangement, we can form a diagonal sub-matrix of size $p_2/\ell$, thereby proving the claim.

%If there is a $1$ entry in two different player's vectors $V(u_1)$ and $V(u_2)$ in the same position $(e,j)$, then this means the number of players using the resource $e$ was changed to $j$ at both time instances. This implies there must be at least one other player who moved to another strategy that changed the number of players using this resource (releasing the resource if it was previously using it, and using it now otherwise), hence this entry was $-1$ in its corresponding move vector, and subsequently (possibly after several such switches) changed to $1$ again in the second player's repeating move. Consider the player that plays some strategy releasing this vector for the last time before its used again by $2$, as $w_{12}$. 
\end{proof}

\begin{lem}\label{lem:cg:prfixedseq}
The probability that a BR sequence $S$ of length $\lambda$ has total improvement in potential at most $\epsilon$ is at most $(\lambda\phi\epsilon)^{p_2/\ell}$, where $p_2$ is the number of repeating players in $S$.
\end{lem}
\begin{proof}
Similar to the proof of Lemma \ref{thm:in-text-qpoly}, the probability of total improvement of the sequence $S$ being at most $\epsilon$, is at most
$$Pr[\sum\limits_{i=1}^\lambda \ip{L_i,C}\in (0,\epsilon)|\ip{L_i,C}>0,\ \forall i]\le Pr[\bigwedge_{i=1}^{p_2/\ell} \ip{V_j,C} \in (0,\epsilon)]\le (\lambda\phi\epsilon)^{p_2/\ell}.$$ 
\end{proof}

We use Definition \ref{def:Delta-l} and Lemma \ref{lem:min-repeating-pairs} to prove Theorem \ref{thm:CGquasipoly}.
 
For an arbitrary BR sequence $S$ of $\lambda$ moves where at least $\lambda/(5log(nk))$ distinct moves appear at least twice, the number of repeating players is at least $\lambda/(5klog(nk))$. By Lemma \ref{lem:cg:prfixedseq} the probability that the total improvement due to $S$ is at most $\epsilon$, is at most $(\lambda\phi\epsilon)^{\lambda/\ell klog(nk)}$.

To find the probability that any sequence is at most $\epsilon$-improving (gives an improvement of at most $\epsilon$), we take a union bound over all possible initial strategy profiles, and all $(nk)^\lambda$ choices of a BR sequence, to get the probability bound
\begin{equation*}
  \begin{split}
Pr[\Delta(\lambda)\in (0,\epsilon)]&\le k^\lambda(nk)^\lambda(\lambda\phi\epsilon)^{p_2/\ell}\\
&\le \left(k(nk)(5nk\phi\epsilon)^{1/5\ell klog(nk)}\right)^{\lambda}\\
&\le \left(2k^3n^2(\phi\epsilon)^{1/5\ell klog(nk)}\right)^{\lambda}
  \end{split}
\end{equation*}
  
  We set $\epsilon=\phi^{-1}(2n^2k^3)^{-2\cdot \ell k log(nk)}$ to get
  $$Pr[\Delta(\lambda)\in (0,\epsilon)]\le \left(\frac{1}{2n^2k^3}\right)^{\lambda}.$$
  Using Lemma \ref{lem:min-repeating-pairs}, we now take a union bound over all choices of $\lambda$ to get:
  $$Pr[\Delta_{5nk}\in (0,\epsilon)]\le \sum\limits_{i=1}^{5nk}(2n^2k^3)^{-\lambda}\le \frac{1}{2n^2k^3-1}.$$
   Hence, with probability $1-1/poly(n,k)$ (over the draw of cost vector $C$), {\em all} BR sequences of length $5nk$ will have total improvement at least $\epsilon$.
In that case, any execution of BR algorithm makes an improvement of at least $\epsilon$ every $5nk$ moves. 

Since the total improvement is at most $2r$, where $r=|E|$, we conclude that the total number of steps is at most $5nk\cdot 2r/\epsilon = 10nkr(2n^2k^3)^{2\ell k\log(nk)}\cdot \phi=
\phi\cdot r(nk)^{O(\ell k\log(nk))}$, and this occurs with probability $1-1/poly(n,k)$.




==> expected_time.tex <==
\begin{thm}\label{thm:expected-time}
Given a PLS problem with input size $N$, potential function range $[-N^{r_1}, N^{r_2}]$, and a local-search algorithm $\mathcal{A}$ to solve it, let $d$ be the number of distinct choices the algorithm has in each step and let $S$ be the total size of the search space of the algorithm. For an instance $I$ drawn at random with density $\phi$. Suppose the probability that any length-$Q$ sequence of improving moves of $\mathcal{A}$ results in total improvement in the potential value at most $\epsilon$ is at most $\sum\limits_{q=1}^Q((\phi N)^{f(N)}(\phi\epsilon)^{1/g(N)})^q$. Here $f(N)$ and $g(N)$ are any functions in $N$. 
Then the expected running-time of the algorithm is $O(g(N)(\phi N)^{f(N)g(N)}lnS)$.
\end{thm}
\begin{proof}
The maximum improvement possible before $\mathcal{A}$ terminates is the maximum change in the potential function value, given by $N^{r_2}+N^{r_1}$. 

For any integer $t\geq 1$, if the algorithm requires more than $t$ steps to terminate, then there must exist some subsequence of length $Q$ that results in an improvement in the potential value of less than $(N^{r_2}+N^{r_1})/t\leq 2N^{max\{r_2,r_1\}}/t$. We denote $r=max\{r_1,r_2\}$.

We define a random variable $T$ as the number of steps $\mathcal{A}$ requires to terminate. Using the notation $\Delta(Q)$ to denote the minimum total improvement in a length $Q$-sequence of the algorithm $\mathcal{A}$, this gives the probability of $\mathcal{A}$ running for more than $t$ steps as:
\begin{equation*}
Pr[T\geq t]\leq Pr[\Delta(Q)\in (0,N^{r}/t)] \leq \sum\limits_{q=1}^Q \left((\phi N)^{f(N)}(\phi\frac{N^r}{t})^{1/g(N)}\right)^q.
\end{equation*}

We define $t=\gamma i$, for $\gamma=(\phi N)^{f(N)g(N)}(\phi N^r)=\phi^{f(N)g(N)+1}N^{f(N)g(N)+r}$, and compute the probability of $T\geq \gamma i$ for any integer $i$:
\begin{equation*}
Pr[T\geq \gamma i]\leq \sum\limits_{q=1}^Q \left((\phi N)^{f(N)}(\phi\frac{N^r}{\gamma i})^{1/g(N)}\right)^q \leq \sum\limits_{q=1}^Q \left(\frac{1}{i}^{q/g(N)}\right) \leq g(N)\frac{1}{i-1}.
\end{equation*}

We now sum over all values of $t$, by using that $Pr[T\geq t]\leq Pr[T\geq t\cdot\lceil t/\gamma \rceil]$, and compute the expected time steps as:
\begin{align*}
E[T]&=\sum_{t=1}^S Pr[T\geq t] \leq \sum_{i=1}^{S}\sum_{t=1}^\gamma Pr[T\geq t\cdot i] \leq \sum_{i=1}^{S}\sum_{t=1}^\gamma Pr[T\geq \gamma i] \leq \sum_{t=1}^\gamma Pr[T\geq \gamma] + \sum_{i=2}^S \frac{g(N)\gamma}{i-1} \\
&\leq \sum_{t=1}^\gamma Pr[T\geq \gamma] + g(N)\gamma ln(S) \leq \gamma +g(N)\gamma ln(S) =O(\gamma g(N)lnS).
\end{align*}

That is, the expected time for $\mathcal{A}$ to terminate is $O(\gamma g(N)lnS)=O(g(N)(\phi N)^{f(N)g(N)}lnS)$.
\end{proof}

\begin{cor}\label{corr:expected-quasi}
The smoothed expected time for BR to terminate for all \nashcoord games is polynomial in $(n^{(klog(nk))},\phi)$.
\end{cor}
\begin{proof}
From Lemma \ref{}, we know that the probability that the minimum improvement in a BR sequence of length $5nk$ is at most $\epsilon$, is at most $$.

Applying theorem \ref{thm:expected-time}, we get $f(N)=O(1)$, and $g(N)=O(klog(nk))$.
\end{proof}

\begin{cor}\label{corr:expected-poly}
For complete graphs, the smoothed expected time for BR to terminate for \nashcoord is 
polynomial in $(n^k,\phi)$.
\end{cor}
\begin{proof}
From Lemma \ref{}, we know that for complete graphs, the probability that the minimum improvement in a BR sequence of length $2nk$ is at most $\epsilon$, is at most $$.

Applying theorem \ref{thm:expected-time}, we get $f(N)=O(1)$, and $g(N)=O(1)$.

\end{proof}





